CMMLoc: Advancing Text-to-PointCloud Localization with Cauchy-Mixture-Model Based Framework

The goal of point cloud localization based on linguistic description is to identify a 3D position using textual description in large urban environments, which has potential applications in various fields, such as determining the location for vehicle pickup or goods delivery. Ideally, for a textual description and its corresponding 3D location, the objects around the 3D location should be fully described in the text description. However, in practical scenarios, e.g., vehicle pickup, passengers usually describe only the part of the most significant and nearby surroundings instead of the entire environment. In response to this $\textbf{partially relevant}$ challenge, we propose $\textbf{CMMLoc}$, an uncertainty-aware $\textbf{C}$auchy-$\textbf{M}$ixture-$\textbf{M}$odel ($\textbf{CMM}$) based framework for text-to-point-cloud $\textbf{Loc}$alization. To model the uncertain semantic relations between text and point cloud, we integrate CMM constraints as a prior during the interaction between the two modalities. We further design a spatial consolidation scheme to enable adaptive aggregation of different 3D objects with varying receptive fields. To achieve precise localization, we propose a cardinal direction integration module alongside a modality pre-alignment strategy, helping capture the spatial relationships among objects and bringing the 3D objects closer to the text modality. Comprehensive experiments validate that CMMLoc outperforms existing methods, achieving state-of-the-art results on the KITTI360Pose dataset. Codes are available in this GitHub repository https://github.com/kevin301342/CMMLoc.

==> sec/06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We analyze existing work on language-based 3D point cloud localization and identify the limitations of the current coarse-to-fine pipeline, namely the neglect of partial relevance between text descriptions and 3D objects and the failure to model this uncertainty. We propose CMMLoc to tackle this problem. In the coarse stage, we are the first to model the task as a partially relevant retrieval problem and propose a Cauchy-Mixture-Model-based Transformer and a spatial consolidation scheme for local modeling of 3D objects and better submap representation. In the fine stage, we enhance fine-grained interactions between texts and objects by pre-aligning text queries with 3D objects and applying a cardinal direction integration module to capture spatial relations between objects. Extensive experiments show that our CMMLoc significantly outperforms the current state-of-the-art, highlighting its effectiveness.
